An integer programming approach for quick-commerce assortment planning

In this paper, we explore the challenge of assortment planning in the context of quick-commerce, a rapidly-growing business model that aims to deliver time-sensitive products. In order to achieve quick delivery to satisfy the immediate demands of online customers in close proximity, personalized online assortments need to be included in brick-and-mortar store offerings. With the presence of this physical linkage requirement and distinct multinomial logit choice models for online consumer segments, the firm seeks to maximize overall revenue by selecting an optimal assortment of products for local stores and by tailoring a personalized assortment for each online consumer segment. We employ an integer programming approach to solve this NP-hard problem to global optimality. In particular, we derive convex hull results to represent the consumer choice of each online segment under a general class of operational constraints, and to characterize the relation between assortment decisions and choice probabilities of products. Our convex hull results, coupled with a modified choice probability ordered separation algorithm, yield formulations that provide a significant computational advantage over existing methods. Finally, we illustrate how our convex hull results can be used to address other assortment optimization problems.

==> Numerical/Table1.tex <==
% Table generated by Excel2LaTeX from sheet 'sh_AGGTABLE'
\begin{table}[H]
\renewcommand\tabcolsep{2pt} % 调整表格列间的长度
\renewcommand{\arraystretch}{1.5} % 调整表格行间高度
\centering
\footnotesize
\caption{Results for problems without ``Luce'' constraints. Instances are randomly repeated 6 times.}
\label{tab:Pref_NoLuce}%
\begin{tabular}{ccccccccccc}
\toprule
\multirow{3}{*}{Models}
          &  {$(n, m) $} 
          & \multicolumn{3}{c}{\textbf{(100, 50)}} 
          & \multicolumn{3}{c}{\textbf{(150, 75)}}
          & \multicolumn{3}{c}{\textbf{(200, 100)}}\\
          \cmidrule{2-11}
          &  $(u_0^{\text{off}}, u_0^{\text{on}})$  
          & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,5)}} & \multicolumn{1}{c}{\textbf{(1,10)}} 
          & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,5)}} & \multicolumn{1}{c}{\textbf{(1,10)}}
          & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,5)}} & \multicolumn{1}{c}{\textbf{(1,10)}} \\
          \midrule
          \textbf{\conic} & \textbf{Nodes} & 37.83  & 315.00  & 388.00  & 26.67  & 363.00  & 679.83  & 115.00  & 848.67  & 1326.67  \\
    \textbf{\our} & \textbf{Nodes} & 1.00  & 1.00  & 1.00  & 1.00  & 2.00  & 11.50  & 1.00  & 11.83  & 11.17  \\
    \textbf{\milp} & \textbf{Nodes} & 337.17  & 4623.00  & 10417.33  & 223.33  & 14951.50  & 29448.00  & 1856.17  & 13271.50  & 13354.83  \\
    \textbf{\conic} & \textbf{Assort} & 34.00  & 43.33  & 51.00  & 42.00  & 56.00  & 66.83  & 50.00  & 63.00  & 77.50  \\
    \textbf{\our} & \textbf{Assort} & 34.00  & 43.67  & 51.17  & 42.67  & 56.17  & 66.67  & 50.83  & 63.17  & 78.33  \\
    \textbf{\milp} & \textbf{Assort} & 34.00  & 43.33  & 51.00  & 42.17  & 56.00  & 66.83  & 50.33  & 63.17  & 77.67  \\
    % \textbf{\conic} & \textbf{NumAssort\_onAvg} & 31.55  & 43.02  & 50.98  & 38.42  & 54.95  & 66.45  & 45.92  & 61.47  & 76.68  \\
    % \textbf{\our} & \textbf{NumAssort\_onAvg} & 31.59  & 43.29  & 51.14  & 38.63  & 55.17  & 66.28  & 46.32  & 61.62  & 77.50  \\
    % \textbf{\milp} & \textbf{NumAssort\_onAvg} & 31.59  & 43.02  & 50.98  & 38.34  & 54.96  & 66.45  & 46.13  & 61.61  & 76.85  \\
    \textbf{\conic} & \textbf{Constrs} & 25502.0  & 25502.0  & 25502.0  & 57002.0  & 57002.0  & 57002.0  & 101002.0  & 101002.0  & 101002.0  \\
    \textbf{\our} & \textbf{Constrs} & 11815.2  & 12665.5  & 13240.5  & 25823.7  & 27981.7  & 29349.8  & 45171.8  & 49411.8  & 51911.0  \\
    \textbf{\milp} & \textbf{Constrs} & 20351.0  & 20351.0  & 20351.0  & 45526.0  & 45526.0  & 45526.0  & 80701.0  & 80701.0  & 80701.0  \\
    \textbf{\conic} & \textbf{\#Solved} & 6.00  & 6.00  & 6.00  & 6.00  & 6.00  & 6.00  & 6.00  & 6.00  & 6.00  \\
    \textbf{\our} & \textbf{\#Solved} & 6.00  & 6.00  & 6.00  & 6.00  & 6.00  & 6.00  & 6.00  & 6.00  & 6.00  \\
    \textbf{\milp} & \textbf{\#Solved} & 6.00  & 6.00  & 6.00  & 6.00  & 5.00  & 1.00  & 6.00  & 4.00  & 0.00  \\
    \textbf{\conic} & \textbf{gap}$\%$ & 0.007  & 0.006  & 0.005  & 0.007  & 0.006  & 0.007  & 0.009  & 0.005  & 0.007  \\
    \textbf{\our} & \textbf{gap$\%$} & 0.001  & 0.003  & 0.004  & 0.003  & 0.003  & 0.003  & 0.002  & 0.003  & 0.007  \\
    \textbf{\milp} & \textbf{gap$\%$} & 0.002  & 0.000  & 0.000  & 0.006  & 0.015  & 0.171  & 0.004  & 0.106  & 0.457  \\
    % \textbf{\conic} & \textbf{ObjVal} & 16.53  & 15.53  & 14.50  & 16.93  & 16.07  & 15.17  & 17.38  & 16.60  & 15.74  \\
    % \textbf{\our} & \textbf{ObjVal} & 16.53  & 15.53  & 14.50  & 16.93  & 16.07  & 15.17  & 17.38  & 16.60  & 15.74  \\
    % \textbf{\milp} & \textbf{ObjVal} & 16.53  & 15.53  & 14.50  & 16.93  & 16.07  & 15.17  & 17.38  & 16.60  & 15.74  \\
    % \textbf{\conic} & \textbf{ObjValLuce} & 16.01  & 15.07  & 14.11  & 16.40  & 15.60  & 14.76  & 16.79  & 16.07  & 15.28  \\
    % \textbf{\our} & \textbf{ObjValLuce} & 16.01  & 15.07  & 14.11  & 16.40  & 15.60  & 14.76  & 16.79  & 16.07  & 15.28  \\
    % \textbf{\milp} & \textbf{ObjValLuce} & 16.01  & 15.07  & 14.11  & 16.40  & 15.60  & 14.76  & 16.79  & 16.07  & 15.28  \\
    \textbf{\conic} 
    & \makecell{\textbf{Time}\\(min)\\(max)} 
    & \makecell{64.14\\(27.78)\\(127.796)}  
    & \makecell{133.92\\(59.15)\\(345.48)}  
    & \makecell{99.13\\(55.14)\\(184.09)}    
    & \makecell{302.32\\(227.03)\\(356.91)} 
    & \makecell{455.81\\(227.42)\\(1212.76)}   
    & \makecell{912.41\\(412.79)\\(1473.12)}   
    & \makecell{415.72\\(191.78)\\(662.64)} 
    & \makecell{1734.78\\(602.56)\\(3431.92)}   
    & \makecell{2999.54\\(1526.15)\\(3578.17)}\\
    \textbf{\our} %& \textbf{Runtime} & 11.00  & 16.59  & 59.30  & 28.60  & 62.16  & 402.61  & 57.99  & 133.81  & 326.93 
    & \makecell{\textbf{Time}\\(min)\\(max)} 
    & \makecell{11.00\\(9.62)\\(12.33)}  
    & \makecell{16.59\\(13.99)\\(25.42)}  
    & \makecell{59.30\\(26.42)\\(85.70)}    
    & \makecell{28.60\\(23.69)\\(33.82)} 
    & \makecell{62.16\\(36.99)\\(115.20)}   
    & \makecell{402.61\\(54.83)\\(764.81)}   
    & \makecell{57.99\\(47.77)\\(77.19)} 
    & \makecell{133.81\\(97.40)\\(254.86)}   
    & \makecell{326.93\\(228.65)\\(413.07)}\\
    \textbf{\milp} 
    % & \textbf{Runtime} & 38.55  & 102.62  & 263.47  & 196.67  & 1199.42  & 3119.01  & 236.76  & 2277.47  & 3600.58  \\
    & \makecell{\textbf{Time}\\(min)\\(max)} 
    & \makecell{39.55\\(14.07)\\(64.82)}  
    & \makecell{102.62\\(38.85)\\(324.77)}  
    & \makecell{263.47\\(119.44)\\(450.96)}    
    & \makecell{196.67\\(96.46)\\(299.46)} 
    & \makecell{1199.42\\(313.14)\\(3600.36)}   
    & \makecell{3119.01\\(712.25)\\(3600.48)}   
    & \makecell{236.76\\(127.31)\\(441.19)} 
    & \makecell{2277.47\\(491.95)\\(3600.42)}   
    & \makecell{3600.58\\(3600.40)\\(3601.05)}\\
    \multirow{2}[0]{*}{\textbf{\our}} & \textbf{Time\_cut} & 9.71  & 12.37  & 54.13  & 24.22  & 35.07  & 318.38  & 48.46  & 74.20  & 95.07  \\
          & \textbf{Time\_sep} & 3.79  & 3.86  & 3.88  & 9.31  & 9.56  & 9.19  & 17.47  & 17.73  & 17.72  \\
    \bottomrule
    \end{tabular}%
\end{table}%


==> Numerical/Table2.tex <==
% Table generated by Excel2LaTeX from sheet 'sh_AGGTABLE'
\begin{table}[H]
\renewcommand\tabcolsep{2pt} % 调整表格列间的长度
\renewcommand{\arraystretch}{1.5} % 调整表格行间高度
\centering
\footnotesize
\caption{Results for problems with ``Luce'' constraints. Instances are randomly repeated 6 times.}
\label{tab:Pref_Luce}%
\begin{tabular}{ccccccccccc}
\toprule
\multirow{3}{*}{Models}
          &  {$(n, m) $} 
          & \multicolumn{3}{c}{\textbf{(100, 50)}} 
          & \multicolumn{3}{c}{\textbf{(150, 75)}}
          & \multicolumn{3}{c}{\textbf{(200, 100)}}\\
          \cmidrule{2-11}
          &  $(u_0^{\text{off}}, u_0^{\text{on}})$  
          & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,5)}} & \multicolumn{1}{c}{\textbf{(1,10)}} 
          & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,5)}} & \multicolumn{1}{c}{\textbf{(1,10)}}
          & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,5)}} & \multicolumn{1}{c}{\textbf{(1,10)}} \\
          \midrule
    \textbf{\conic} & \textbf{Nodes} & 191.83  & 1547.67  & 835.50  & 14409.00  & 22165.17  & 15777.83  & 13837.33  & 1844.17  & 1414.67  \\
    \textbf{\our} & \textbf{Nodes} & 1.00  & 1.00  & 1.00  & 1.00  & 1.00  & 18.33  & 1.00  & 1.00  & 2.83  \\
    \textbf{MILP} & \textbf{Nodes} & 342570.50  & 237707.00  & 164130.17  & 145382.33  & 57762.17  & 18971.83  & 20904.83  & 16144.00  & 8297.50  \\
    \textbf{\conic} & \textbf{Assort} & 34.00  & 43.67  & 51.33  & 42.67  & 56.33  & 67.67  & 50.33  & 63.83  & 78.33  \\
    \textbf{\our} & \textbf{Assort} & 34.00  & 44.17  & 51.67  & 42.83  & 56.83  & 67.83  & 50.50  & 64.50  & 79.00  \\
    \textbf{MILP} & \textbf{Assort} & 34.00  & 43.67  & 51.33  & 42.67  & 56.33  & 67.67  & 50.50  & 64.00  & 78.83  \\
    % \textbf{\conic} & \textbf{Assort\_onAvg} & 26.75  & 36.10  & 42.57  & 32.64  & 45.90  & 55.64  & 38.43  & 51.27  & 63.36  \\
    % \textbf{\our} & \textbf{Assort\_onAvg} & 26.75  & 36.50  & 42.85  & 32.69  & 46.27  & 55.79  & 38.41  & 51.70  & 64.03  \\
    % \textbf{MILP} & \textbf{Assort\_onAvg} & 26.75  & 36.10  & 42.57  & 32.63  & 45.90  & 55.65  & 38.47  & 51.39  & 63.83  \\
    \textbf{\conic} & \textbf{Constrs} & 34009.2  & 34009.2  & 34009.2  & 81679.2  & 81679.2  & 81679.2  & 156217.7  & 156217.7  & 156217.7  \\
    \textbf{\our} & \textbf{Constrs} & 20207.7  & 21298.7  & 22033.2  & 50568.2  & 53210.8  & 54235.8  & 100373.3  & 103946.2  & 107238.8  \\
    \textbf{MILP} & \textbf{Constrs} & 28858.2  & 28858.2  & 28858.2  & 70203.2  & 70203.2  & 70203.2  & 135916.7  & 135916.7  & 135916.7  \\
    \textbf{\conic} & \textbf{\#Solved} & 6.00  & 6.00  & 6.00  & 5.00  & 3.00  & 5.00  & 0.00  & 0.00  & 0.00  \\
    \textbf{\our} & \textbf{\#Solved} & 6.00  & 6.00  & 6.00  & 6.00  & 6.00  & 6.00  & 6.00  & 6.00  & 6.00  \\
    \textbf{MILP} & \textbf{\#Solved} & 1.00  & 0.00  & 0.00  & 0.00  & 0.00  & 0.00  & 0.00  & 0.00  & 0.00  \\
    \textbf{\conic} & \textbf{gap} & 0.009  & 0.009  & 0.007  & 0.010  & 0.011  & 0.010  & 0.023  & 0.120  & 0.249  \\
    \textbf{\our} & \textbf{gap} & 0.001  & 0.003  & 0.005  & 0.001  & 0.003  & 0.004  & 0.001  & 0.006  & 0.007  \\
    \textbf{MILP} & \textbf{gap} & 0.037  & 0.064  & 0.114  & 0.079  & 0.225  & 0.530  & 0.138  & 0.436  & 0.859  \\
    % \textbf{\conic} & \textbf{ObjVal} & 16.49  & 15.48  & 14.43  & 16.90  & 16.02  & 15.10  & 17.35  & 16.54  & 15.67  \\
    % \textbf{\our} & \textbf{ObjVal} & 16.49  & 15.48  & 14.43  & 16.90  & 16.02  & 15.10  & 17.35  & 16.54  & 15.67  \\
    % \textbf{MILP} & \textbf{ObjVal} & 16.49  & 15.48  & 14.43  & 16.90  & 16.02  & 15.10  & 17.35  & 16.54  & 15.67  \\
    % \textbf{\conic} & \textbf{ObjValLuce} & 16.49  & 15.48  & 14.43  & 16.90  & 16.02  & 15.10  & 17.35  & 16.54  & 15.67  \\
    % \textbf{\our} & \textbf{ObjValLuce} & 16.49  & 15.48  & 14.43  & 16.90  & 16.02  & 15.10  & 17.35  & 16.54  & 15.67  \\
    % \textbf{MILP} & \textbf{ObjValLuce} & 16.49  & 15.48  & 14.43  & 16.90  & 16.02  & 15.10  & 17.35  & 16.54  & 15.67  \\
    \textbf{\conic} 
    % & \textbf{Time} & 172.27  & 451.33  & 541.72  & 1568.93  & 2710.67  & 2706.11  & 3600.71  & 3604.57  & 3618.38  \\
    & \makecell{\textbf{Time}\\(min)\\(max)} 
    & \makecell{172.27\\(61.85)\\(345.82)}  
    & \makecell{451.33\\(247.72)\\(590.75)}  
    & \makecell{541.72\\(293.01)\\(751.24)}    
    & \makecell{1568.93\\(859.56)\\(3600.48)} 
    & \makecell{2710.67\\(1306.46)\\(3600.64)}   
    & \makecell{2706.11\\(1341.31)\\(3600.46)}   
    & \makecell{3600.71\\(3600.55)\\(3600.83)} 
    & \makecell{3604.57\\(3600.40)\\(3623.10)}   
    & \makecell{3618.38\\(3600.78)\\(3653.99)}\\
    \textbf{\our} 
    % & \textbf{Time} & 13.28  & 20.87  & 36.28  & 46.70  & 92.91  & 140.53  & 130.78  & 208.14  & 518.67  \\
    & \makecell{\textbf{Time}\\(min)\\(max)} 
    & \makecell{13.28\\(11.72)\\(15.28)}  
    & \makecell{20.87\\(16.77)\\(30.62)}  
    & \makecell{36.28\\(27.14)\\(54.05)}    
    & \makecell{46.70\\(39.86)\\(52.12)} 
    & \makecell{92.91\\(61.66)\\(155.80)}   
    & \makecell{140.53\\(96.59)\\(232.20)}   
    & \makecell{130.78\\(120.65)\\(160.50)} 
    & \makecell{208.14\\(171.85)\\(298.45)}   
    & \makecell{518.67\\(287.14)\\(1182.69)}\\
    \textbf{MILP} 
    % & \textbf{Time} & 3034.57  & 3600.79  & 3600.82  & 3600.43  & 3619.71  & 3613.61  & 3614.65  & 3629.31  & 3602.13  \\
    & \makecell{\textbf{Time}\\(min)\\(max)} 
    & \makecell{3034.57\\(205.08)\\(3600.57)}  
    & \makecell{3600.79\\(3600.40)\\(3601.72)}  
    & \makecell{3600.82\\(3600.31)\\(3602.19)}    
    & \makecell{3600.43\\(3600.29)\\(3600.65)} 
    & \makecell{3619.71\\(3600.21)\\(3675.44)}   
    & \makecell{3613.61\\(3600.36)\\(3630.07)}   
    & \makecell{3614.65\\(3600.88)\\(3637.58)} 
    & \makecell{3629.31\\(3600.50)\\(3664.38)}   
    & \makecell{3602.13\\(3600.39)\\(3608.25)}\\
    \multirow{2}[0]{*}{\textbf{\our}} 
          & \textbf{Time\_cut} & 11.63  & 15.36  & 25.35  & 39.92  & 55.18  & 59.28  & 110.48  & 134.20  & 165.72  \\
          & \textbf{Time\_sep} & 3.79  & 3.92  & 4.07  & 9.32  & 9.47  & 9.57  & 16.02  & 16.20  & 16.99  \\
    \multirow{2}[0]{*}{\textbf{Luce} }
        & \textbf{\#paths} & \#paths  & \#paths  & \#paths  & \#paths  & \#paths  & \#paths  & \#paths  & \#paths  & \#paths  \\
        & \textbf{depth} & depth  & depth  & depth  & depth  & depth  & depth  & depth  & depth  & depth  \\
        % & \makecell{\textbf{paths}\\\textbf{depths}} 
        % & \makecell{paths\\depths} 
        % & \makecell{paths\\depths} 
        % & \makecell{paths\\depths}   
        % & \makecell{paths\\depths} 
        % & \makecell{paths\\depths} 
        % & \makecell{paths\\depths} 
        % & \makecell{paths\\depths} 
        % & \makecell{paths\\depths}   
        % & \makecell{paths\\depths} \\
    \bottomrule
    \end{tabular}%
\end{table}%


==> Numerical/Table_cmp.tex <==
% Table generated by Excel2LaTeX from sheet 'sh_AGGTABLE'
\begin{table}[H]
\renewcommand\tabcolsep{2pt} % 调整表格列间的宽度
\renewcommand{\arraystretch}{1.2} % 调整表格行间高度
\centering
\footnotesize
\caption{Results for problems for the case without Luce constraints (``No Luce'') and with constraints (``Luce''). Instances are randomly repeated 6 times.}
\label{tab:Pref_NoLuce}%
\begin{tabular}{cccccccccccc}
\toprule
\multirow{2}{*}{\makecell{\textbf{Luce}\\\textbf{Constr.}} }
& \multirow{2}{*}{\textbf{Formul.}}
          &  {$(n, m) $} 
          & \multicolumn{3}{c}{\textbf{(100, 50)}} 
          & \multicolumn{3}{c}{\textbf{(150, 75)}}
          & \multicolumn{3}{c}{\textbf{(200, 100)}}\\
          \cmidrule{3-12}
          &   &  $(u_0^{\text{off}}, u_0^{\text{on}})$  
          & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,5)}} & \multicolumn{1}{c}{\textbf{(1,10)}} 
          & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,5)}} & \multicolumn{1}{c}{\textbf{(1,10)}}
          & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,5)}} & \multicolumn{1}{c}{\textbf{(1,10)}} \\
          \midrule
    \multirow{11}[0]{*}{\textbf{\makecell{No\\Luce}} } 
    &   \textbf{\our} 
        & \makecell{\textbf{Time}\\(min)\\(max)} 
        & \makecell{11.0\\(9.6)\\(12.3)}  
        & \makecell{16.5\\(13.9)\\(25.4)}  
        & \makecell{59.3\\(26.4)\\(85.7)}    
        & \makecell{28.6\\(23.6)\\(33.8)} 
        & \makecell{62.1\\(36.9)\\(115.2)}   
        & \makecell{402.6\\(54.8)\\(764.8)}   
        & \makecell{57.9\\(47.7)\\(77.1)} 
        & \makecell{133.8\\(97.4)\\(254.8)}   
        & \makecell{326.9\\(228.6)\\(413.0)}\\
    &   \textbf{\conic} 
        & \makecell{\textbf{Time}\\(min)\\(max)} 
        & \makecell{64.1\\(27.7)\\(127.7)}  
        & \makecell{133.9\\(59.15)\\(345.4)}  
        & \makecell{99.1\\(55.1)\\(184.0)}    
        & \makecell{302.3\\(227.0)\\(356.9)} 
        & \makecell{455.8\\(227.4)\\(1212.7)}   
        & \makecell{912.4\\(412.7)\\(1473.1)}   
        & \makecell{415.7\\(191.7)\\(662.6)} 
        & \makecell{1734.7\\(602.5)\\(3431.9)}   
        & \makecell{2999.5\\(1526.1)\\(3578.1)}\\
    &   \textbf{\milp} 
        & \makecell{\textbf{Time}\\(min)\\(max)} 
        & \makecell{39.5\\(14.1)\\(64.8)}  
        & \makecell{102.6\\(38.8)\\(324.7)}  
        & \makecell{263.4\\(119.4)\\(450.9)}    
        & \makecell{196.6\\(96.4)\\(299.4)} 
        & \makecell{1199.4\\(313.1)\\(3600.3)}   
        & \makecell{3119.1\\(712.2)\\(3600.4)}   
        & \makecell{236.7\\(127.3)\\(441.1)} 
        & \makecell{2277.4\\(491.9)\\(3600.4)}   
        & \makecell{3600.5\\(3600.4)\\(3601.0)}\\
    &   \textbf{\our} & \textbf{Nodes} & 1.0  & 1.0  & 1.0  & 1.0  & 2.0  & 11.5  & 1.0  & 11.8  & 11.1  \\
    &   \textbf{\conic} & \textbf{Nodes} & 37.8  & 315.0  & 388.0  & 26.6  & 363.0  & 679.8  & 115.0  & 848.6  & 1326.67  \\
    &   \textbf{\milp} & \textbf{Nodes} & 337.1  & 4623.0  & 10417.3  & 223.3  & 14951.5  & 29448.0  & 1856.2  & 13271.5  & 13354.8  \\
    &   \textbf{\our} & \textbf{\#Solved} & 6  & 6  & 6  & 6  & 6  & 6  & 6  & 6  & 6  \\
    &   \textbf{\conic} & \textbf{\#Solved} & 6  & 6  & 6  & 6  & 6  & 6  & 6  & 6  & 6  \\
    &   \textbf{\milp} & \textbf{\#Solved} & 6  & 6  & 6  & 6  & 5  & 1  & 6  & 4  & 0  \\
    &   \multicolumn{2}{c}{\textbf{Cutting Time}} 
        & 9.7  & 12.3  & 54.1  & 24.2  & 35.1  & 318.3  & 48.4  & 74.2  & 95.1  \\
    &   \multicolumn{2}{c}{\textbf{Separation Time}} 
    & 3.7  & 3.8  & 3.8  & 9.3  & 9.5  & 9.1  & 17.4  & 17.7  & 17.8  \\
    % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \midrule
    \multirow{11}[0]{*}{\textbf{Luce} }
    &   \textbf{\our} 
        & \makecell{\textbf{Time}\\(min)\\(max)} 
        & \makecell{13.2\\(11.7)\\(15.2)}  
        & \makecell{20.8\\(16.7)\\(30.6)}  
        & \makecell{36.2\\(27.1)\\(54.1)}    
        & \makecell{46.7\\(39.8)\\(52.1)} 
        & \makecell{92.9\\(61.6)\\(155.8)}   
        & \makecell{140.5\\(96.5)\\(232.2)}   
        & \makecell{130.7\\(120.6)\\(160.5)} 
        & \makecell{208.1\\(171.8)\\(298.4)}   
        & \makecell{518.6\\(287.1)\\(1182.6)}\\
    &   \textbf{\conic} 
        & \makecell{\textbf{Time}\\(min)\\(max)} 
        & \makecell{172.2\\(61.8)\\(345.8)}  
        & \makecell{451.3\\(247.7)\\(590.7)}  
        & \makecell{541.7\\(293.0)\\(751.2)}    
        & \makecell{1568.9\\(859.5)\\(3600.4)} 
        & \makecell{2710.6\\(1306.4)\\(3600.6)}   
        & \makecell{2706.1\\(1341.3)\\(3600.4)}   
        & \makecell{3600.7\\(3600.5)\\(3600.8)} 
        & \makecell{3604.5\\(3600.4)\\(3623.1)}   
        & \makecell{3618.3\\(3600.7)\\(3653.9)}\\
    &   \textbf{\milp} 
        & \makecell{\textbf{Time}\\(min)\\(max)} 
        & \makecell{3034.5\\(205.0)\\(3600.5)}  
        & \makecell{3600.7\\(3600.4)\\(3601.7)}  
        & \makecell{3600.8\\(3600.3)\\(3602.1)}    
        & \makecell{3600.4\\(3600.2)\\(3600.6)} 
        & \makecell{3619.7\\(3600.2)\\(3675.4)}   
        & \makecell{3613.6\\(3600.3)\\(3630.1)}   
        & \makecell{3614.6\\(3600.8)\\(3637.5)} 
        & \makecell{3629.3\\(3600.5)\\(3664.3)}   
        & \makecell{3602.1\\(3600.3)\\(3608.2)}\\
    &   \textbf{\our} & \textbf{Nodes} & 1.0  & 1.0  & 1.0  & 1.0  & 1.0  & 18.3  & 1.0  & 1.0  & 2.8  \\
    &   \textbf{\conic} & \textbf{Nodes} & 191.8  & 1547.6  & 835.5  & 14409.0  & 22165.1  & 15777.8  & 13837.3  & 1844.1  & 1414.6  \\
    &   \textbf{\milp} & \textbf{Nodes} & 342570.5  & 237707.0  & 164130.1  & 145382.3  & 57762.1  & 18971.8  & 20904.8  & 16144.0  & 8297.5  \\
    &   \textbf{\our} & \textbf{\#Solved} & 6  & 6  & 6  & 6  & 6  & 6  & 6  & 6  & 6  \\
    &   \textbf{\conic} & \textbf{\#Solved} & 6  & 6  & 6  & 5  & 3  & 5  & 0  & 0  & 0  \\
    &   \textbf{\milp} & \textbf{\#Solved} & 1  & 0  & 0  & 0  & 0  & 0  & 0  & 0  & 0  \\
    &   \multicolumn{2}{c}{\textbf{Cutting Time}} 
        & 11.6  & 15.3  & 25.3  & 39.9  & 55.1  & 59.2  & 110.4  & 134.2  & 165.7  \\
    &   \multicolumn{2}{c}{\textbf{Separation Time}} 
        & 3.7  & 3.9  & 4.0  & 9.3  & 9.4  & 9.5  & 16.0  & 16.2  & 16.9  \\
\bottomrule
\end{tabular}%
\end{table}%




% % Table generated by Excel2LaTeX from sheet 'sh_AGGTABLE'
% \begin{table}[H]
% \renewcommand\tabcolsep{2pt} % 调整表格列间的长度
% \renewcommand{\arraystretch}{1.5} % 调整表格行间高度
% \centering
% \footnotesize
% \caption{Results for problems with ``Luce'' constraints. Instances are randomly repeated 6 times.}
% \label{tab:Pref_Luce}%
% \begin{tabular}{ccccccccccc}
% \toprule
% \multirow{3}{*}{Models}
%           &  {$(n, m) $} 
%           & \multicolumn{3}{c}{\textbf{(100, 50)}} 
%           & \multicolumn{3}{c}{\textbf{(150, 75)}}
%           & \multicolumn{3}{c}{\textbf{(200, 100)}}\\
%           \cmidrule{2-11}
%           &  $(u_0^{\text{off}}, u_0^{\text{on}})$  
%           & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,5)}} & \multicolumn{1}{c}{\textbf{(1,10)}} 
%           & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,5)}} & \multicolumn{1}{c}{\textbf{(1,10)}}
%           & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,5)}} & \multicolumn{1}{c}{\textbf{(1,10)}} \\
%           \midrule
% \cmidrule{1-11}
%     \textbf{\our} & \textbf{Nodes} & 1.0  & 1.0  & 1.0  & 1.0  & 1.0  & 18.3  & 1.0  & 1.0  & 2.8  \\
%     \textbf{\conic} & \textbf{Nodes} & 191.8  & 1547.6  & 835.5  & 14409.0  & 22165.1  & 15777.8  & 13837.3  & 1844.1  & 1414.6  \\
%     \textbf{\milp} & \textbf{Nodes} & 342570.5  & 237707.0  & 164130.1  & 145382.3  & 57762.1  & 18971.8  & 20904.8  & 16144.0  & 8297.5  \\
%     \textbf{\our} & \textbf{\#Solved} & 6  & 6  & 6  & 6  & 6  & 6  & 6  & 6  & 6  \\
%     \textbf{\conic} & \textbf{\#Solved} & 6  & 6  & 6  & 5  & 3  & 5  & 0  & 0  & 0  \\
%     \textbf{\milp} & \textbf{\#Solved} & 1  & 0  & 0  & 0  & 0  & 0  & 0  & 0  & 0  \\
%     \textbf{\our} 
%     & \makecell{\textbf{Time}\\(min)\\(max)} 
%     & \makecell{13.2\\(11.7)\\(15.2)}  
%     & \makecell{20.8\\(16.7)\\(30.6)}  
%     & \makecell{36.2\\(27.1)\\(54.1)}    
%     & \makecell{46.7\\(39.8)\\(52.1)} 
%     & \makecell{92.9\\(61.6)\\(155.8)}   
%     & \makecell{140.5\\(96.5)\\(232.2)}   
%     & \makecell{130.7\\(120.6)\\(160.5)} 
%     & \makecell{208.1\\(171.8)\\(298.4)}   
%     & \makecell{518.6\\(287.1)\\(1182.6)}\\
%     \textbf{\conic} 
%     & \makecell{\textbf{Time}\\(min)\\(max)} 
%     & \makecell{172.2\\(61.8)\\(345.8)}  
%     & \makecell{451.3\\(247.7)\\(590.7)}  
%     & \makecell{541.7\\(293.0)\\(751.2)}    
%     & \makecell{1568.9\\(859.5)\\(3600.4)} 
%     & \makecell{2710.6\\(1306.4)\\(3600.6)}   
%     & \makecell{2706.1\\(1341.3)\\(3600.4)}   
%     & \makecell{3600.7\\(3600.5)\\(3600.8)} 
%     & \makecell{3604.5\\(3600.4)\\(3623.1)}   
%     & \makecell{3618.3\\(3600.7)\\(3653.9)}\\
%     \textbf{\milp} 
%     & \makecell{\textbf{Time}\\(min)\\(max)} 
%     & \makecell{3034.5\\(205.0)\\(3600.5)}  
%     & \makecell{3600.7\\(3600.4)\\(3601.7)}  
%     & \makecell{3600.8\\(3600.3)\\(3602.1)}    
%     & \makecell{3600.4\\(3600.2)\\(3600.6)} 
%     & \makecell{3619.7\\(3600.2)\\(3675.4)}   
%     & \makecell{3613.6\\(3600.3)\\(3630.1)}   
%     & \makecell{3614.6\\(3600.8)\\(3637.5)} 
%     & \makecell{3629.3\\(3600.5)\\(3664.3)}   
%     & \makecell{3602.1\\(3600.3)\\(3608.2)}\\
%     \multicolumn{2}{c}{\textbf{Cutting Time}} 
%         & 11.6  & 15.3  & 25.3  & 39.9  & 55.1  & 59.2  & 110.4  & 134.2  & 165.7  \\
%     \multicolumn{2}{c}{\textbf{Separation Time}} 
%         & 3.7  & 3.9  & 4.0  & 9.3  & 9.4  & 9.5  & 16.0  & 16.2  & 16.9  \\
%     \multicolumn{2}{c}{\textbf{Luce: \#paths}} 
%         & \#paths  & \#paths  & \#paths  & \#paths  & \#paths  & \#paths  & \#paths  & \#paths  & \#paths  \\
%     \multicolumn{2}{c}{\textbf{Luce: depth}} 
%         & depth  & depth  & depth  & depth  & depth  & depth  & depth  & depth  & depth  \\
%     % \multirow{2}[0]{*}{\textbf{\our}} 
%     %       & \textbf{Time\_cut} & 11.63  & 15.36  & 25.35  & 39.92  & 55.18  & 59.28  & 110.48  & 134.20  & 165.72  \\
%     %       & \textbf{Time\_sep} & 3.79  & 3.92  & 4.07  & 9.32  & 9.47  & 9.57  & 16.02  & 16.20  & 16.99  \\
%     % \multirow{2}[0]{*}{\textbf{Luce} }
%     %     & \textbf{\#paths} & \#paths  & \#paths  & \#paths  & \#paths  & \#paths  & \#paths  & \#paths  & \#paths  & \#paths  \\
%     %     & \textbf{depth} & depth  & depth  & depth  & depth  & depth  & depth  & depth  & depth  & depth  \\
% \bottomrule
% \end{tabular}%
% \end{table}%


==> Numerical/table_cmp_0717.tex <==
% Table generated by Excel2LaTeX from sheet 'sh_AGGTABLE'
\begin{table}[H]
\renewcommand\tabcolsep{2pt} % 调整表格列间的宽度
\renewcommand{\arraystretch}{1.2} % 调整表格行间高度
\centering
\footnotesize
\caption{Results for problems for the case without Luce constraints (``No Luce'') and with constraints (``Luce''). Instances are randomly repeated 24 times.}
\label{tab:Pref_NoLuce}%
\begin{threeparttable}   
\begin{tabular}{cccccccccccc}
\toprule
\multirow{2}{*}{\makecell{\textbf{Luce}\\\textbf{Constr.}} }
& \multirow{2}{*}{\textbf{Formul.}}
          &  {$(n, m) $} 
          & \multicolumn{3}{c}{\textbf{(100, 50)}} 
          & \multicolumn{3}{c}{\textbf{(150, 75)}}
          & \multicolumn{3}{c}{\textbf{(200, 100)}}\\
          \cmidrule{3-12}
          &   &  $(u_0^{\text{off}}, u_0^{\text{on}})$  
          & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,5)}} & \multicolumn{1}{c}{\textbf{(1,10)}} 
          & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,5)}} & \multicolumn{1}{c}{\textbf{(1,10)}}
          & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,5)}} & \multicolumn{1}{c}{\textbf{(1,10)}} \\
          \midrule
		\multirow{20}[0]{*}{\makecell{\textbf{No}\\\textbf{Luce}}} & \multirow{4}[0]{*}{\textbf{SPR-ip}} & \textbf{Time} & 7.9   & 14.7  & 28.3  & 20.4  & 43.8  & 174.4  & 44.0  & 84.9  & 471.9  \\
		   &       & \textbf{min} & 6.0   & 6.6   & 10.0  & 15.1  & 23.1  & 38.4  & 29.8  & 59.7  & 142.8  \\
		   &       & \textbf{max} & 11.0  & 44.0  & 80.7  & 25.9  & 173.8  & 378.8  & 79.1  & 184.5  & 1827.0  \\
		   &       & \textbf{std} & 1.5   & 10.3  & 15.5  & 3.4   & 30.6  & 77.1  & 11.0  & 24.2  & 382.0  \\
		   & \multirow{4}[0]{*}{\textbf{Conic}} & \textbf{Time} & 63.9  & 97.7  & 157.4  & 306.3  & 493.4  & 916.6  & 662.8  & 1916.6  & 3190.1  \\
		   &       & \textbf{min} & 5.7   & 36.5  & 56.0  & 121.0  & 216.5  & 346.5  & 342.2  & 742.1  & 2024.8  \\
		   &       & \textbf{max} & 240.2  & 296.6  & 402.5  & 494.1  & 2034.9  & 1736.0  & 3162.5  & 3600.0  & 3600.0  \\
		   &       & \textbf{std}\tnote{i} & 50.1  & 59.3  & 100.9  & 94.7  & 396.1  & 395.5  & 562.0  & --  & --  \\
		   & \multirow{4}[0]{*}{\textbf{MILP}} & \textbf{Time} & 36.5  & 105.7  & 535.5  & 200.8  & 1019.9  & 3121.0  & 212.6  & 3204.8  & 3601.3  \\
		   &       & \textbf{min} & 3.4   & 17.1  & 50.6  & 39.4  & 141.2  & 793.1  & 85.9  & 1658.2  & 3600.0  \\
		   &       & \textbf{max} & 140.0  & 611.4  & 3600.0  & 439.1  & 3600.0  & 3600.0  & 414.5  & 3600.0  & 3600.0  \\
		   &       & \textbf{std} & 34.4  & 123.0  & --  & 105.0  & --  & --  & 89.7  & --  & --  \\
		   & \textbf{SPR-ip} & \textbf{\#Solved} & 24  & 24  & 24  & 24  & 24  & 24  & 24  & 24  & 24  \\
		   & \textbf{Conic} & \textbf{\#Solved} & 24  & 24  & 24  & 24  & 24  & 24  & 24  & 20  & 12  \\
		   & \textbf{MILP} & \textbf{\#Solved} & 24  & 24  & 23  & 24  & 21  & 8   & 24  & 9   & 0  \\
		   & \textbf{SPR-ip} & \textbf{Nodes} & 1.0   & 1.0   & 3.7   & 1.0   & 3.6   & 5.2   & 1.0   & 1.0   & 89.2  \\
		   & \textbf{Conic} & \textbf{Nodes} & 21.1  & 253.4  & 475.0  & 49.1  & 494.9  & 699.2  & 170.5  & 821.2  & 1038.1  \\
		   & \textbf{MILP} & \textbf{Nodes} & 423.5  & 4369.0  & 20349.9  & 684.8  & 10879.6  & 27539.5  & 1049.0  & 13105.3  & 11099.2  \\
		   & \multicolumn{2}{c}{\textbf{Cutting\_Time}\tnote{ii}}  & 6.3   & 10.1  & 16.6  & 15.3  & 18.3  & 103.9  & 30.8  & 38.1  & 92.1  \\
		   % & \multicolumn{2}{c}{\textbf{Separation\_Time}\tnote{ii}}  & 3.8   & 3.9   & 3.9   & 9.0   & 9.1   & 9.0   & 17.0  & 17.3  & 17.6  \\
		\midrule
		\multirow{20}[1]{*}{\textbf{Luce}} & \multirow{4}[1]{*}{\textbf{SPR-ip}} & \textbf{Time} & 8.9   & 17.1  & 29.0  & 30.6  & 63.5  & 132.4  & 83.0  & 161.1  & 564.4  \\
		   &       & \textbf{min} & 6.9   & 9.2   & 14.8  & 22.5  & 33.0  & 63.8  & 58.5  & 96.9  & 155.0  \\
		   &       & \textbf{max} & 13.7  & 38.8  & 74.8  & 39.1  & 156.1  & 301.8  & 106.3  & 229.6  & 2150.1  \\
		   &       & \textbf{std} & 1.6   & 7.1   & 14.1  & 4.3   & 29.9  & 67.0  & 13.7  & 37.3  & 439.1  \\
		   & \multirow{4}[0]{*}{\textbf{Conic}} & \textbf{Time} & 310.3  & 531.9  & 622.3  & 1901.8  & 2925.1  & 2746.8  & 3459.6  & 3600.0  & 3600.0  \\
		   &       & \textbf{min} & 32.9  & 149.2  & 290.7  & 332.4  & 853.8  & 1249.5  & 2281.9  & 3600.0  & 3600.0  \\
		   &       & \textbf{max} & 3600.0  & 1250.6  & 1874.0  & 3600.0  & 3600.0  & 3600.0  & 3600.0  & 3600.0  & 3600.0  \\
		   &       & \textbf{std} & --  & 241.0  & 347.6  & --  & --  & --  & --  & --  & --  \\
		   & \multirow{4}[0]{*}{\textbf{MILP}} & \textbf{Time} & 3049.1  & 3600.0  & 3600.0  & 3600.0  & 3600.0  & 3600.0  & 3600.0  & 3600.0  & 3600.0  \\
		   &       & \textbf{min} & 72.9  & 3600.0  & 3600.0  & 3600.0  & 3600.0  & 3600.0  & 3600.0  & 3600.0  & 3600.0  \\
		   &       & \textbf{max} & 3600.0  & 3600.0  & 3600.0  & 3600.0  & 3600.0  & 3600.0  & 3600.0  & 3600.0  & 3600.0  \\
		   &       & \textbf{std} & --  & --   & --   & --   & --  & --  & --  & --  & --  \\
		   & \textbf{SPR-ip} & \textbf{\#Solved} & 24  & 24  & 24  & 24  & 24  & 24  & 24  & 24  & 24  \\
		   & \textbf{Conic} & \textbf{\#Solved} & 23  & 24  & 24  & 19  & 11  & 17  & 5   & 0   & 0  \\
		   & \textbf{MILP} & \textbf{\#Solved} & 4   & 0   & 0   & 0   & 0   & 0   & 0   & 0   & 0  \\
		   & \textbf{SPR-ip} & \textbf{Nodes} & 1.0   & 1.0   & 34.6  & 1.0   & 7.1   & 22.4  & 1.0   & 2.6   & 139.7  \\
		   & \textbf{Conic} & \textbf{Nodes} & 7726.8  & 2776.5  & 1837.3  & 27123.9  & 13932.2  & 9836.1  & 8015.5  & 1607.0  & 1653.0  \\
		   & \textbf{MILP} & \textbf{Nodes} & 342460.4  & 195369.7  & 138716.1  & 131540.7  & 49869.5  & 18491.5  & 28618.0  & 10923.9  & 6552.6  \\
		   & \multicolumn{2}{c}{\textbf{Cutting\_Time}} & 7.1   & 8.6   & 12.4  & 22.7  & 27.7  & 30.8  & 59.2  & 71.2  & 80.1  \\
		   % & \multicolumn{2}{c}{\textbf{Separation\_Time}} & 3.7   & 3.8   & 3.9   & 9.2   & 9.2   & 9.4   & 16.3  & 16.7  & 16.8  \\
    \bottomrule
\end{tabular}%
\begin{tablenotes}
\footnotesize
\item[i]
    The \textbf{std} is omitted (denoted by ``--'') if not all $24$ instances are solved successfully.
\item[ii]
    The \textbf{Cutting\_Time} denotes the time for generating cuts before solving the final IP problem. 
% \item[ii] 
    % The \textbf{Separation\_Time} denotes the time consumed by the separation process (Algorithm \ref{alg:sep}), which has been included in \textbf{Cutting\_Time}.
\end{tablenotes}
\end{threeparttable}
\end{table}%



==> Numerical/table_cmp_0729.tex <==
% Table generated by Excel2LaTeX from sheet 'sh_AGGTABLE'
\begin{table}[htbp]
	\renewcommand\tabcolsep{2.5pt} % 调整表格列间的宽度
	\renewcommand{\arraystretch}{0.75} % 调整表格行间高度	
        \centering
	\footnotesize
	\caption{Computational performance comparison }
	\label{tab:Pref_NoLuce_Luce}%
	\begin{threeparttable}   
		\begin{tabular}{ccccccccccc}
			\toprule
			\multirow{2}{*}{\textbf{Formul.}}
			&  {$(n, m) $} 
			& \multicolumn{3}{c}{\textbf{(100, 50)}} 
			& \multicolumn{3}{c}{\textbf{(150, 75)}}
			& \multicolumn{3}{c}{\textbf{(200, 100)}}\\
			\cmidrule{2-11}
			&  $(u_0^{\text{off}}, u_0^{\text{on}})$  
			& \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,5)}} & \multicolumn{1}{c}{\textbf{(1,10)}} 
			& \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,5)}} & \multicolumn{1}{c}{\textbf{(1,10)}}
			& \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,5)}} & \multicolumn{1}{c}{\textbf{(1,10)}} \\
			\midrule
			  \multirow{4}[0]{*}{\textbf{CH-2}} & \textbf{Time} & 1.6   & 4.7   & 11.7  & 5.5   & 28.9  & 79.7  & 13.6  & 156.0  & 448.6  \\
			& \textbf{min} & 0.4   & 0.8   & 1.8   & 1.7   & 5.1   & 17.0  & 3.9   & 18.1  & 71.0  \\
			& \textbf{max} & 5.3   & 26.2  & 50.8  & 15.7  & 153.0  & 250.6  & 46.8  & 3358.0  & 2014.2  \\
			& \textbf{std} & 1.2   & 5.7   & 11.2  & 2.7   & 30.9  & 62.1  & 9.7   & 554.1  & 458.4  \\
                & \textbf{Nodes} & 1.0   & 1.0   & 3.0   & 1.0   & 3.0   & 15.8  & 1.0   & 95.3  & 101.8  \\
                & \textbf{Solved} & 36    & 36    & 36    & 36    & 36    & 36    & 36    & 36    & 36  \\
			\multirow{4}[0]{*}{\textbf{Conic}} & \textbf{Time} & 75.8  & 120.8  & 190.6  & 347.5  & 583.9  & 1040.3  & 744.8  & 2189.1  & 3286.3  \\
			& \textbf{min} & 5.7   & 36.5  & 56.0  & 121.0  & 216.5  & 346.5  & 297.4  & 683.9  & 2024.8  \\
			& \textbf{max} & 240.2  & 588.8  & 490.9  & 845.9  & 2034.9  & 2430.9  & 3600  & 3600  & 3600  \\
			& {\textbf{std}} & 48.7  & 96.4  & 127.7  & 146.0  & 430.9  & 531.5  & --  & --  & -- \\
                & \textbf{Nodes} & 14.4  & 219.6  & 482.3  & 44.1  & 506.3  & 752.2  & 166.7  & 718.7  & 892.4  \\
                & \textbf{Solved} & 36    & 36    & 36    & 36    & 36    & 36    & 35    & 24    & 17  \\
			 \multirow{4}[0]{*}{\textbf{MILP}} & \textbf{Time} & 46.8  & 131.8  & 663.6  & 251.2  & 1190.9  & 3169.8  & 329.2  & 3225.4  & 3600  \\
			& \textbf{min} & 3.4   & 17.1  & 50.6  & 39.4  & 141.2  & 793.1  & 85.9  & 1658.2  & 3600  \\
			& \textbf{max} & 175.9  & 611.4  & 3600  & 544.5  & 3600  & 3600  & 3241.6  & 3600  & 3600  \\
			& \textbf{std} & 42.2  & 131.9  & --  & 132.3  & --  & --  & 519.1  & --  & --  \\
                & \textbf{Nodes} & 411.2  & 3732.6  & 19321.2  & 577.0  & 10686.7  & 23726.2  & 1493.4  & 12141.4  & 9841.4  \\
                & \textbf{Solved} & 36    & 36    & 35    & 36    & 31    & 10    & 36    & 13    & 0  \\
			% \textbf{CH-2} & \textbf{Nodes} & 1.0   & 1.0   & 3.0   & 1.0   & 3.0   & 15.8  & 1.0   & 95.3  & 101.8  \\
			% \textbf{Conic} & \textbf{Nodes} & 14.4  & 219.6  & 482.3  & 44.1  & 506.3  & 752.2  & 166.7  & 718.7  & 892.4  \\
			% \textbf{MILP} & \textbf{Nodes} & 411.2  & 3732.6  & 19321.2  & 577.0  & 10686.7  & 23726.2  & 1493.4  & 12141.4  & 9841.4  \\
			% \textbf{CH-2} & \textbf{Solved} & 36    & 36    & 36    & 36    & 36    & 36    & 36    & 36    & 36  \\
			% \textbf{Conic} & \textbf{Solved} & 36    & 36    & 36    & 36    & 36    & 36    & 35    & 24    & 17  \\
			% \textbf{MILP} & \textbf{Solved} & 36    & 36    & 35    & 36    & 31    & 10    & 36    & 13    & 0  \\
			\multicolumn{2}{c}{\textbf{Alg. 2 running time}}& 6.6   & 10.4  & 16.9  & 16.0  & 19.4  & 112.0  & 31.8  & 40.7  & 95.9  \\
			% & \textbf{SeparationTime} & 4.0   & 4.1   & 4.1   & 9.5   & 9.6   & 9.6   & 17.9  & 18.4  & 18.6  \\
        \midrule
			 \multirow{4}[0]{*}{\textbf{CH-Chain-2}} 
                & \textbf{Time} & 2.0   & 8.7   & 18.2  & 8.4   & 40.3  & 113.0  & 26.3  & 184.4  & 608.4  \\
			  & \textbf{min} & 0.6   & 1.2   & 3.3   & 3.3   & 9.9   & 30.0  & 7.4   & 44.1  & 66.4  \\
			& \textbf{max} & 6.3   & 34.4  & 62.1  & 16.1  & 140.0  & 271.0  & 119.3  & 3052.2  & 3469.3  \\
			& \textbf{std} & 1.3   & 7.7   & 14.5  & 3.1   & 32.7  & 79.3  & 18.1  & 495.1  & 638.9  \\
                & \textbf{Nodes} & 411.2  & 3732.6  & 19321.2  & 577.0  & 10686.7  & 23726.2  & 1493.4  & 12141.4  & 9841.4  \\
                & \textbf{Solved} & 36    & 36    & 36    & 36    & 36    & 36    & 36    & 36    & 36  \\
			\multirow{4}[0]{*}{\textbf{Conic-Chain}} & \textbf{Time} & 335.4  & 551.2  & 709.4  & 2130.7  & 2948.4  & 2837.1  & 3510.1  & 3600  & 3600  \\
			& \textbf{min} & 32.9  & 149.2  & 290.7  & 332.4  & 853.8  & 1249.5  & 2281.9  & 3600  & 3600  \\
			& \textbf{max} & 3600  & 1250.6  & 1874.0  & 3600  & 3600 & 3600  & 3600  & 3600  & 3600  \\
			& \textbf{std} & --  & 227.7  & 345.1  & --  & --  & --  & --  & --  & --  \\
                & \textbf{Nodes} & 5234.4  & 2628.8  & 2201.3  & 25308.7  & 12792.8  & 8082.9  & 7338.2  & 1546.8  & 1507.6  \\
                & \textbf{Solved} & 35    & 36    & 36    & 28    & 16    & 25    & 5     & 0     & 0  \\
			\multirow{4}[0]{*}{\textbf{MILP-Chain}} & \textbf{Time} & 3233.0  & 3600  & 3600  & 3600  & 3600  & 3600  & 360  & 3600  & 3600  \\
			& \textbf{min} & 72.9  & 3600  & 3600  & 3600  & 3600  & 3600  & 3600  & 3600  & 3600  \\
			& \textbf{max} & 3600  & 3600  & 3600  & 3600  & 3600  & 3600  & 3600  & 3600  & 3600  \\
			& \textbf{std} & --  & --   & --   & --   & --  & --   & --  & --  & --  \\
                & \textbf{Nodes} & 308996.9  & 182801.1  & 113729.0  & 105800.7  & 45419.9  & 16591.3  & 25915.5  & 10538.1  & 5426.1  \\
                & \textbf{Solved} & 4     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0  \\
			% \textbf{CH-Chain-2} & \textbf{Nodes} & 1.0   & 1.4   & 25.2  & 1.0   & 10.2  & 38.2  & 1.0   & 109.7  & 162.9  \\
			% \textbf{Conic-Chain} & \textbf{Nodes} & 5234.4  & 2628.8  & 2201.3  & 25308.7  & 12792.8  & 8082.9  & 7338.2  & 1546.8  & 1507.6  \\
			% \textbf{MILP-Chain} & \textbf{Nodes} & 308996.9  & 182801.1  & 113729.0  & 105800.7  & 45419.9  & 16591.3  & 25915.5  & 10538.1  & 5426.1  \\
			% \textbf{CH-Chain-2}  & \textbf{Solved} & 36    & 36    & 36    & 36    & 36    & 36    & 36    & 36    & 36  \\
			% \textbf{Conic-Chain} & \textbf{Solved} & 35    & 36    & 36    & 28    & 16    & 25    & 5     & 0     & 0  \\
			% \textbf{MILP-Chain} & \textbf{Solved} & 4     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0  \\
			\multicolumn{2}{c}{\textbf{Alg. 2 running time}} & 7.5   & 9.1   & 12.9  & 23.4  & 29.0  & 31.8  & 60.1  & 71.9  & 83.4  \\
%			&       & \textbf{SeparationTime} & 3.9   & 4.0   & 4.1   & 9.7   & 9.8   & 9.9   & 17.5  & 17.8  & 18.0  \\
			\bottomrule
		\end{tabular}%
		% \begin{tablenotes}
		% 	\footnotesize
		% 	% \item[i]
		% 	% The \textbf{std} is omitted (denoted by ``--'') if not all 3636 instances are solved successfully.
		% 	% \item[i]
		% 	% The \textbf{Cut generation time}
  %  % denotes the time for generating cuts before solving the final integer problems. That is the time consumed by Algorithm ????????????????????????????????????\ref{alg:cutting} when K=2K=2.
		% 	% \item[ii] 
		% 	% The \textbf{Separation\_Time} denotes the time consumed by the separation process (Algorithm ????????????????????????????????????\ref{alg:sep}), which has been included in \textbf{Cutting\_Time}.
		% \end{tablenotes}
	\end{threeparttable}
\end{table}%



==> Numerical/table_result_for_sparseVIP_largeScale.tex <==
% Table generated by Excel2LaTeX from sheet 'sh_AGGTABLE'
\begin{table}[H]
\renewcommand\tabcolsep{2pt} % 调整表格列间的长度
\renewcommand{\arraystretch}{0.9}
\centering
\footnotesize
\caption{Results for problems with sparse attractive value and discount price ($U[0.8,1]$) for each online segment without extra constraint.}
\label{tab:sparseVIP_large}%
\begin{tabular}{ccccccccccc}
\toprule
\multirow{3}{*}{Models}
          &  {$(|{M}|, |{N}|) $} 
          & \multicolumn{3}{c}{\textbf{(100, 100)}} 
          & \multicolumn{3}{c}{\textbf{(200, 100)}}
          & \multicolumn{3}{c}{\textbf{(500, 100)}}\\
          \cmidrule{2-11}
          &  $(v_0^{off}, v_0^{on})$  
          & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,2)}} 
          & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,2)}}
          & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,2)}} & \multicolumn{1}{c}{\textbf{(1,2)}} \\
          \cmidrule{2-11}
          & $(s^{off}, s^{on})$  
          & \multicolumn{1}{c}{\textbf{(1,0.1)}} & \multicolumn{1}{c}{\textbf{(1,0.5)}} & \multicolumn{1}{c}{\textbf{(1,1)}} 
          & \multicolumn{1}{c}{\textbf{(1,0.1)}} & \multicolumn{1}{c}{\textbf{(1,0.5)}} & \multicolumn{1}{c}{\textbf{(1,1)}}
          & \multicolumn{1}{c}{\textbf{(1,0.1)}} & \multicolumn{1}{c}{\textbf{(1,0.5)}} & \multicolumn{1}{c}{\textbf{(1,1)}}\\
          \midrule
        \textbf{Conic\_Conic} & \textbf{NodeCount} & 407   & 170   & 321   & 1070  & 2558  & 905   & 2383  & 463   & 179 \\
    \textbf{Conic\_Conv} & \textbf{NodeCount} & 3644  & 830   & 431   & 205406 & 221156 & 28046 & 376861 & 203738 & 63292 \\
    \textbf{MC\_Conv} & \textbf{NodeCount} & 97606 & 2954  & 867   & 1989837 & 538481 & 29655 & 578627 & 255341 & 73167 \\
    \textbf{MC\_Conv-aC} & \textbf{NodeCount} & 1     & 1     & 1     & 142   & 110   & 1     & 107557 & 248   & 5377 \\
    \textbf{MC\_Conv-mo} & \textbf{NodeCount} & 82515 & 2858  & 673   & 1973204 & 597727 & 25715 & 587785 & 255873 & 73301 \\
    \textbf{MC\_Conv-mo-aC} & \textbf{NodeCount} & 1     & 1     & 1     & 1     & 83    & 1     & 143162 & 105   & 5057 \\
    \textbf{MC\_MC} & \textbf{NodeCount} & 95639 & 5579  & 3336  & 1031679 & 191704 & 49378 & 248739 & 25041 & 15686 \\
    \midrule
    \textbf{Conic\_Conic} & \textbf{NumAssort} & 58    & 45    & 33    & 112   & 69    & 57    & 165   & 112   & 95 \\
    \textbf{Conic\_Conv} & \textbf{NumAssort} & 58    & 45    & 33    & 112   & 69    & 57    & 166   & 112   & 95 \\
    \textbf{MC\_Conv} & \textbf{NumAssort} & 58    & 45    & 33    & 112   & 69    & 57    & 165   & 113   & 94 \\
    \textbf{MC\_Conv-aC} & \textbf{NumAssort} & 58    & 44    & 34    & 112   & 69    & 57    & 165   & 112   & 95 \\
    \textbf{MC\_Conv-mo} & \textbf{NumAssort} & 58    & 45    & 33    & 112   & 69    & 57    & 165   & 113   & 93 \\
    \textbf{MC\_Conv-mo-aC} & \textbf{NumAssort} & 58    & 44    & 34    & 112   & 68    & 56    & 165   & 113   & 95 \\
    \textbf{MC\_MC} & \textbf{NumAssort} & 58    & 45    & 33    & 112   & 69    & 57    & 165   & 113   & 95 \\
    \midrule
    \textbf{Conic\_Conic} & \textbf{NumConstrs} & 50602 & 50602 & 50602 & 101002 & 101002 & 101002 & 252202 & 252202 & 252202 \\
    \textbf{Conic\_Conv} & \textbf{NumConstrs} & 20502 & 20502 & 20502 & 40902 & 40902 & 40902 & 102102 & 102102 & 102102 \\
    \textbf{MC\_Conv} & \textbf{NumConstrs} & 20501 & 20501 & 20501 & 40901 & 40901 & 40901 & 102101 & 102101 & 102101 \\
    \textbf{MC\_Conv-aC} & \textbf{NumConstrs} & 21795 & 22683 & 22565 & 42825 & 44421 & 44230 & 106077 & 106490 & 108110 \\
    \textbf{MC\_Conv-mo} & \textbf{NumConstrs} & 20501 & 20501 & 20501 & 40901 & 40901 & 40901 & 102101 & 102101 & 102101 \\
    \textbf{MC\_Conv-mo-aC} & \textbf{NumConstrs} & 21625 & 22606 & 22520 & 42811 & 44341 & 44113 & 105982 & 106451 & 108046 \\
    \textbf{MC\_MC} & \textbf{NumConstrs} & 50501 & 50501 & 50501 & 100901 & 100901 & 100901 & 252101 & 252101 & 252101 \\
    \midrule
    \textbf{Conic\_Conic} & \textbf{NumSolved} & 1     & 1     & 1     & 1     & 1     & 0     & 0     & 0     & 0 \\
    \textbf{Conic\_Conv} & \textbf{NumSolved} & 1     & 1     & 1     & 1     & 1     & 1     & 0     & 0     & 0 \\
    \textbf{MC\_Conv} & \textbf{NumSolved} & 1     & 1     & 1     & 0     & 0     & 1     & 0     & 0     & 0 \\
    \textbf{MC\_Conv-aC} & \textbf{NumSolved} & 1     & 1     & 1     & 1     & 1     & 1     & 0     & 1     & 1 \\
    \textbf{MC\_Conv-mo} & \textbf{NumSolved} & 1     & 1     & 1     & 0     & 0     & 1     & 0     & 0     & 0 \\
    \textbf{MC\_Conv-mo-aC} & \textbf{NumSolved} & 1     & 1     & 1     & 1     & 1     & 1     & 0     & 1     & 1 \\
    \textbf{MC\_MC} & \textbf{NumSolved} & 1     & 1     & 1     & 0     & 0     & 1     & 0     & 0     & 0 \\
    \midrule
    \textbf{Conic\_Conic} & \textbf{Runtime} & 167.472  & 80.569  & 93.853  & 778.397  & 3308.012  & 3600.164  & 3600.370  & 3652.843  & 3600.199  \\
    \textbf{Conic\_Conv} & \textbf{Runtime} & 11.672  & 6.231  & 8.016  & 480.409  & 1504.724  & 333.935  & 3600.436  & 3600.223  & 3600.706  \\
    \textbf{MC\_Conv} & \textbf{Runtime} & 116.790  & 13.271  & 12.173  & 3600.107  & 3600.199  & 332.411  & 3600.298  & 3600.160  & 3600.363  \\
    \textbf{MC\_Conv-aC} & \textbf{Runtime} & 3.986  & 9.168  & 10.044  & 15.588  & 36.633  & 38.028  & 3638.499  & 150.474  & 1161.877  \\
    \textbf{MC\_Conv-mo} & \textbf{Runtime} & 99.513  & 11.710  & 10.520  & 3600.117  & 3600.196  & 270.730  & 3600.432  & 3600.211  & 3600.376  \\
    \textbf{MC\_Conv-mo-aC} & \textbf{Runtime} & 3.778  & 9.513  & 11.033  & 14.092  & 46.822  & 38.348  & 3637.194  & 138.972  & 1372.473  \\
    \textbf{MC\_MC} & \textbf{Runtime} & 264.739  & 79.998  & 101.898  & 3600.299  & 3600.302  & 2838.401  & 3600.583  & 3600.256  & 3600.427  \\
    \midrule
    \textbf{Conic\_Conic} & \textbf{gap} & 0.010  & 0.009  & 0.007  & 0.008  & 0.005  & 0.042  & 0.332  & 0.304  & 0.327  \\
    \textbf{Conic\_Conv} & \textbf{gap} & 0.000  & 0.000  & 0.000  & 0.009  & 0.010  & 0.004  & 0.786  & 0.193  & 0.261  \\
    \textbf{MC\_Conv} & \textbf{gap} & 0.000  & 0.000  & 0.000  & 0.242  & 0.087  & 0.003  & 1.098  & 0.239  & 0.261  \\
    \textbf{MC\_Conv-aC} & \textbf{gap} & 0.004  & 0.007  & 0.007  & 0.008  & 0.000  & 0.004  & 0.028  & 0.007  & 0.009  \\
    \textbf{MC\_Conv-mo} & \textbf{gap} & 0.006  & 0.000  & 0.000  & 0.220  & 0.083  & 0.000  & 1.077  & 0.238  & 0.258  \\
    \textbf{MC\_Conv-mo-aC} & \textbf{gap} & 0.008  & 0.007  & 0.004  & 0.010  & 0.008  & 0.007  & 0.032  & 0.006  & 0.009  \\
    \textbf{MC\_MC} & \textbf{gap} & 0.000  & 0.004  & 0.000  & 0.271  & 0.164  & 0.008  & 1.139  & 0.310  & 0.313  \\
    \bottomrule
    \end{tabular}%
\end{table}%

